PALMED: Throughput Characterization for Superscalar Architectures -- Extended Version

In a super-scalar architecture, the scheduler dynamically assigns micro-operations ($\mu$OPs) to execution ports. The port mapping of an architecture describes how an instruction decomposes into $\mu$OPs and lists for each $\mu$OP the set of ports it can be mapped to. It is used by compilers and performance debugging tools to characterize the performance throughput of a sequence of instructions repeatedly executed as the core component of a loop. This paper introduces a dual equivalent representation: The resource mapping of an architecture is an abstract model where, to be executed, an instruction must use a set of abstract resources, themselves representing combinations of execution ports. For a given architecture, finding a port mapping is an important but difficult problem. Building a resource mapping is a more tractable problem and provides a simpler and equivalent model. This paper describes Palmed, a tool that automatically builds a resource mapping for pipelined, super-scalar, out-of-order CPU architectures. Palmed does not require hardware performance counters, and relies solely on runtime measurements. We evaluate the pertinence of our dual representation for throughput modeling by extracting a representative set of basic-blocks from the compiled binaries of the SPEC CPU 2017 benchmarks. We compared the throughput predicted by existing machine models to that produced by Palmed, and found comparable accuracy to state-of-the art tools, achieving sub-10 % mean square error rate on this workload on Intel's Skylake microarchitecture.

==> artifact.tex <==
\subsection{Description}
The artifact provides the user with all the files needed in a Dockerfile and a docker images. All experimental requirements and the basic run steps are provided in the following sections, but the complete walk-through  of \tool used is described {in the project's README} (\url{https://gitlab.inria.fr/nderumig/palmed/}) and on the artifacts' README (\url{https://gitlab.inria.fr/CORSE/palmed-artifact}).

\subsubsection{How delivered}
The artifact is two-fold: a Dockerfile is available {on INRIA's GitLab} (\url{https://gitlab.inria.fr/CORSE/palmed-artifact}), as well as a precompiled Docker image (\url{https://gitlab.inria.fr/CORSE/palmed-artifact/container_registry/1338}). Moreover, \tool is distributed under the GNU GPLv3 license and its source code is also available on the same GitLab (\url{https://gitlab.inria.fr/nderumig/palmed/}). The docker image's size is about 2 GiB and is not expected to significantly increase during runtime. 

\subsubsection{Hardware dependencies}
Our experimental setup includes an Intel Skylake-SP CPU (Intel Xeon Silver 4114) and a first-generation AMD Zen processor (AMD EPYC 7401P), that are needed to exactly reproduce our experimental section. They can be offered from \href{https://scaleway.com}{Scaleway}, but there is no strict constraint on that: \tool can run on any recent x86 system from both Intel and AMD. However, a high core count is preferable to reduce benchmarking and solving time, with took in total less than 11 hours on our test machines.

Moreover, Simultaneous Multi-Threading (SMT) \emph{must} be disabled, either directly in the BIOS or is performed automatically in our Docker image, and no other task should run on the benchmarking machine. We also require a high RAM capacity (32 GiB should be fine, but this requirement increase with the number of cores available).

\subsubsection{Software dependencies}
\tool requires a valid license of the {Gurobi} (\url{https://www.gurobi.com/}) solver (Academic version is possible).

The system should run a Linux OS with \texttt{perf\_event\_paranoid} set to 1 for access to performance counters (the process is described in the \texttt{README}).

Intel's Architecture Code Analyzer (IACA) (\url{https://www.intel.com/content/www/us/en/developer/articles/tool/architecture-code-analyzer.html}) is proprietary and required for its evaluation with \tool, it can be freely download on Intel's webpage (\url{https://www.intel.com/content/www/us/en/developer/articles/tool/architecture-code-analyzer-download.html}).

All other dependencies are embedded in the docker image. We used Linux Kernel 4.19 and PAPI 6.0.0.1 for our experiments, but this is not a hard requirement as we do not expect our results to significantly differ with software updates.

\subsubsection{Data Sets}
Our evaluation uses microbenchmarks extracted from the SPECrate CPU 2017 benchmark suite. As this benchmark suite is proprietary, we cannot provide free access to this code; however, we would be happy to offer access to it for evaluation purposes through a third-party canal.

The other microbenchmark suite used, PolyBench/C, is embedded in the Docker image.

\subsection{Installation}

Prefer to follow the more extensive instructions from the artifacts's README (\url{https://gitlab.inria.fr/CORSE/palmed-artifact}) if needed, for instance in order to rebuild the docker image or to have more details on the scripts usage.

The command to download the docker image is:\\
\texttt{docker pull registry.gitlab.inria.fr/ corse/palmed-artifact/palmed:v1.0}

Then run the Docker image with:\\
\texttt{docker run --init --privileged --shm-size=1g --cap-add=cap\_sys\_nice --security-opt seccomp=seccomp.json -it --env GUROBI\_KEY=[...] --name=palmed palmed registry.gitlab.inria.fr/ corse/palmed-artifact/palmed:v1.0}

Note that:
\begin{itemize}
\item It is necessary to run the Docker container with the capability \texttt{cap\_sys\_nice} enabled (\texttt{--cap-add=cap\_sys\_nice}); else, \tool won't be able to set the scheduler to FIFO mode and pin processes to cores while running benchmarks.
\item The \texttt{--security-opt seccomp=seccomp.json} changes which syscalls are blocked.
Our file is based on the default as of now, with the \texttt{perf\_event\_open} syscall allowed (don't trust us, diff the files). This is required to use \texttt{libpapi} and read the CPU cycles elapsed.
\item For the same reasons of lower-level access, it is necessary to pass the
\texttt{--privileged} flag.
\item The \texttt{--shm-size=1g} increases the shared memory available to the container. Without this, requests to the database will fail.
\item You must provide a Gurobi license key through the \texttt{GUROBI\_KEY} environment variable, which can be obtained here for academic purposes. If you would rather skip this step, you can pass the value SKIP, but \tool will not work unless you manually register your license later.
\end{itemize}

\subsection{Experiment workflow}
The artifact enables you to reproduce our experiments to various extents (the detailed commands are described in the dockerfile's README):
\begin{itemize}
\item \texttt{only-aggregate}: take for granted the produced model and evaluation benchmarks, simply aggregate the results and compute metrics.
For instance: \texttt{palmed-reproduce-only-aggregate.sh SKX}

\item \texttt{only-evaluate}: take for granted the produced model, but re-evaluate it on basic blocks and derive metrics.
For instance: \texttt{palmed-reproduce-only-evaluate.sh SKX}

\item \texttt{trust-db}: take for granted the produced microbenchmarks, but derive a model from those. Be careful, as \tool's model derivation algorithm can ask for more
benchmark at all times. Given that Gurobi (our solver) is not deterministic,
even though Palmed completed once with those exact provided microbenchmarks,
there is no guarantee that \tool will not compute more benchmarks anyway.
For instance: \texttt{palmed-reproduce-trust-db.sh SKX}

\item \texttt{reproduce-everything}: re-compute everything from scratch.
For instance: \texttt{palmed-reproduce-everything.sh SKX}
\end{itemize}


\subsection{Evaluation and expected result}
Every provided script described on the former section should output Root-Mean-Square error and Kendall's Tau values matching the ones reported in Fig.~\ref{tab:realcpu_results} as terminal-text tables. The only difference between the scripts relies in the number of steps reproduced / taken from our own experiments.

\subsection{Experiment customization}
Any x86 CPU is supported by \tool by running our artifact with the \texttt{reproduce-everything}. However, comparisons with other tool is susceptible to be incorrect depending on their own support of the targeted architecture.

Microbenchmarks customization for evaluation is possible but not trivial, as no documentation is currently provided for this format. However, we do provide a web demo (\url{https://palmed.corse.inria.fr/}), on which throughput predictions are directly output from raw assembly code.

